S2HPruner: Soft-to-Hard Distillation Bridges the Discretization Gap in Pruning

Recently, differentiable mask pruning methods optimize the continuous relaxation architecture (soft network) as the proxy of the pruned discrete network (hard network) for superior sub-architecture search. However, due to the agnostic impact of the discretization process, the hard network struggles with the equivalent representational capacity as the soft network, namely discretization gap, which severely spoils the pruning performance. In this paper, we first investigate the discretization gap and propose a novel structural differentiable mask pruning framework named S2HPruner to bridge the discretization gap in a one-stage manner. In the training procedure, SH2Pruner forwards both the soft network and its corresponding hard network, then distills the hard network under the supervision of the soft network. To optimize the mask and prevent performance degradation, we propose a decoupled bidirectional knowledge distillation. It blocks the weight updating from the hard to the soft network while maintaining the gradient corresponding to the mask. Compared with existing pruning arts, S2HPruner achieves surpassing pruning performance without fine-tuning on comprehensive benchmarks, including CIFAR-100, Tiny ImageNet, and ImageNet with a variety of network architectures. Besides, investigation and analysis experiments explain the effectiveness of S2HPruner. Codes will be released soon.

==> sections/backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccclccl@{}}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Reconstruction}                            &  & \multicolumn{2}{c}{Generation}        \\ \cmidrule(lr){2-4} \cmidrule(l){6-7} 
                        & MPJPE $\downarrow$ & PAMPJPE$\downarrow$ & ACCL$\downarrow$ &  & FID$\downarrow$& DIV$\rightarrow$\\ \midrule
Real  &  \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}& \multicolumn{1}{c}{-} & &  $0.002\hidden{^{\pm.000}}$&	$9.503\hidden{^{\pm.065}}$     \\ \midrule
VPoser-t~\cite{vposer_SMPL-X:2019}  & $75.6$ & $48.6$& $9.3$ &     & $1.430\hidden{^{\pm.002}}$ & $8.336\hidden{^{\pm.099}}$   \\
ACTOR~\cite{petrovich21actor}     & $65.3$ & $41.0$& $7.0$ &     & $0.341\hidden{^{\pm.002}}$ & $9.569\hidden{^{\pm.099}}$ \\
 \midrule
% 7 256
\textbf{Ours-7} ($\mathcal{V}$,skip,9 layers) & $\boldsymbol{14.7}$ & $ \boldsymbol{8.9}$ & $\boldsymbol{5.1}$ &  & $\boldsymbol{0.017}\hidden{^{\pm.000}}$ &  $\boldsymbol{9.554}\hidden{^{\pm.062}}$  \\
\toprule
\toprule
$\mathcal{V}$-1 ($z$,$\mathbb{R}^{1\times256}$) & $54.4$ & $41.6$ & $8.3$ &  & $0.247\hidden{^{\pm.001}}$ & $9.630\hidden{^{\pm.081}}$ \\
Ours-2 ($z$,$\mathbb{R}^{2\times256}$) & $51.8$ & $37.8$ & $8.3$ &  & $0.166\hidden{^{\pm.001}}$ &  $9.626\hidden{^{\pm.087}}$ \\
Ours-5 ($z$,$\mathbb{R}^{5\times256}$) & $24.3$ & $14.7$ & $5.8$ &  & $0.043\hidden{^{\pm.000}}$ & $9.593\hidden{^{\pm.084}}$ \\
Ours-7 ($z$,$\mathbb{R}^{7\times256}$) & $14.7$ & $ 8.9$ & $5.1$ &  & $0.017\hidden{^{\pm.000}}$ &  $9.554\hidden{^{\pm.062}}$\\
Ours-10 ($z$,$\mathbb{R}^{10\times256}$) & $17.3$ & $11.5$ &  $5.8$  && $0.025\hidden{^{\pm.000}}$ & $9.589\hidden{^{\pm.090}}$  \\
\midrule
Ours-7 ($\mathcal{V}$,w/ skip) & $14.7$ & $ 8.9$ & $5.1$ &  & $0.017\hidden{^{\pm.000}}$ & $9.554\hidden{^{\pm.062}}$   \\
Ours-7 ($\mathcal{V}$, w/o skip) &$18.5$ & $10.4$ & $5.6$ && $0.027\hidden{^{\pm.000}}$ & $9.528\hidden{^{\pm.067}}$ &  \\
\midrule
Ours-7 ($\mathcal{V}$, 7 layers) & $16.0$ & $10.2$ & $5.3$ && $0.022\hidden{^{\pm.000}}$ &  $9.593\hidden{^{\pm.075}}$ \\
Ours-7 ($\mathcal{V}$, 9 layers) &$14.7$ & $ 8.9$ & $5.1$ &  & $0.017\hidden{^{\pm.000}}$ & $9.554\hidden{^{\pm.062}}$  \\
Ours-7 ($\mathcal{V}$, 11 layers) & $17.2$& $11.2$ & $5.4$ && $0.021\hidden{^{\pm.000}}$ &  $9.533\hidden{^{\pm.092}}$ & \\ \bottomrule
\end{tabular}%
}
\vspace{2pt}
\caption{Evaluation of our VAE models $\mathcal{V}$ on the motion part of HumanML3D~\cite{Guo_2022_CVPR_humanml3d} dataset: MPJPE and PAMPJPE are measured in millimeter. ACCL indicates acceleration error. We evaluate FID and DIV the same as \cref{tab:tm:comp:humanml3d}. From top to down, we propose real reference, VPoser-t~\cite{vposer_SMPL-X:2019} and ACTOR~\cite{petrovich21actor} as baselines, the evaluation on latent $z\in\mathbb{R}^{i\times256}$, with (w/) or without (w/o) skip connection, $\mathcal{V}$ with different number of transformer layers.}
\label{tab:mr:ablation}
\end{table}


More recently, two categories of motion synthesis methods have emerged: 1) joint latent spaces~\cite{petrovich22temos, ahuja2019language2pose} and 2) diffusion models~\cite{zhang2022motiondiffuse, mdm2022human, kim2022flame}.
%
% 尝试再增加几篇同样的joint latent文章
The former category, like TEMOS~\cite{petrovich22temos}, proposes a variational autoencoder (VAE) architecture to \lw{learn a joint latent space of motion and text, which is constrained on a Gaussian distribution. (wait for modification)}
% 多模态数据 本身结构和分布高度不对齐
However, these multi-modal data, particularly textual descriptions and motion sequence, \cx{has} a quite misaligned structure and different distribution, \lw{which is too difficult to uniform their distribution into one sharing Gaussian distribution. (wait for modification)}
%
Although many previous works~\cite{petrovich21actor, motionvae_ling2020character} have verified that VAE can generate plausible motions just with latent vectors, the cross-modal training could still downgrade motion quality and diversity.
% At same time, action category

Influenced by the great success of the diffusion models~\cite{imagen_saharia2022photorealistic, stable_diffusion} on image synthesis, \cite{mdm2022human, zhang2022motiondiffuse} propose motion diffusion models to learn the relation between motion and input conditions, like text distribution, and generate plausible results.
% 有稍微一些误差的
However, diffusion models are not very applicable to raw motion data with potential noise and temporal-consistency redundancy, thus easily causing \cx{slightly misdirected} distribution by the outliers. \lw{In addition, directly applying the diffusion model to the raw motion data suffers from high computational overheads and low inference speed.}








% 1 multi-model inputs and generative
%
Motion generative models allow human motion synthesis from multi-model inputs, 
%
Although motion generative models, like Variational AutoEncoders (VAE)~\cite{petrovich21actor,motionvae_ling2020character, guo2020action2motion} and Generative Adversarial Networks (GAN)~\cite{lin2018human, ahn2018text2action}, can enable effective human motion sampling,
%
% recent works\cite{ldm-2-28-54, temos-16-42} recommend that VAEs are more \cx{easier to train or training friendly} compared to GANs. Following this suggestion, we employ VAEs in our neural network architectures.
%
recent studies~\cite{arjovsky2017wasserstein, gulrajani2017improved, guo2020action2motion, petrovich21actor} recommend VAEs rather than GANs since the latter are more difficult to train.
%
We thus follow their suggestion.


% 4 motion synthesis: 1 unconstrained generation 2 conditioned synthesis: text-conditioned, action-conditioned
Considering human motion synthesis has enormous condition inputs, here we focus on three typical tasks: 1) unconstrained generation~\cite{xx, vposer_SMPL-X:2019},
%
% 基于直接manual-crafted的motion representaion, neural
Based on \cx{manual-crafted} motion representation, latent representation are widely used in neural operations, xxx
%
Vposer xx for single pose
%
xxxactor used, motionVAE, use latent representation for motion
%
GAN motion ??
%
2) text input~\cite{petrovich22temos, mdm2022human} and 3) action inputs~\cite{petrovich21actor, guo2020action2motion}.
% unconstrained generation
For unconstrained generation, xxx
% The human motion manifold can also be learned without labels, as shown by Holden et al. (2016),
% V-Poser (Pavlakos et al., 2019), and more recently the dedicated MoDi architecture (Raab et al.,
% 2022). We show that our model is capable for such an unsupervised setting as well.
%
% Text-conditioned Motion Synthesis
%
To solve text-to-motion task, the cross-modal approaches~\cite{petrovich22temos, ahuja2019language2pose} learn to share the latent space between language and motion.
%
JL2P~\cite{ahuja2019language2pose} autoencoder
%
temos and t2m tm2m xx vae    temost, Text2Action
%
%
MotionCLIP~\cite{tevet2022motionclip}.
%
To solve action-to-motion task, xxx
% 
xxxx
% 指
A key limitation of many mentioned state-of-the-art motion generation models is a \cx{bad for domain transfer?}, which need re-designed or re-train the whole network for other tasks.
% 
While our models decouple the motion generation models and condition embedding models, we can leverage large motion dataset, like AMASS, to learn a more plausible motion generator.
% summary: Compare to vae based, more application, better robust to text, xx
Therefore, we can easily apply different conditions inputs under same motion generator, like text description and action category.


% \iffalse
% % 2 dataset, motion representation, latent representation
%     %% dataset
%     KIT humanML dataset, babel action-languagle
%     % motion representation
%     joints position, smpl rotation, features, ...
%     %% latent representation
%     VAE - actor, temos 1x256, others  Action2Motion 
%     GAN?
% \fi
%
% 删减一些
The marker-based and markless motion capture approaches~\cite{VIBE_CVPR2020, wan2021encoder, he2021challencap, chen2021sportscap} collect large plausible data for human motion synthesis.
%
While the motion-only AMASS datasets\cite{AMASS_ICCV2019} and its extended datasets benefit multi-model motion generation tasks, such as KIT Motion-Lanugage dataset~\cite{Plappert2016kit} and HumanML3d~\cite{Guo_2022_CVPR_humanml3d} with text description, Babel~\cite{BABEL:CVPR:2021} with action category, and xx with,
%
they also lead to the \cx{discussions or issues or questions} on motion representation.
% ??
% the most straightforward motion representaion is joint position.
%
Based on the SMPL model, the classical and widely-used motion representation \cite{VIBE_CVPR2020, chen2021sportscap} in motion capture is decoupled shape $\mathbf{\beta}$ and pose parameters $\mathbf{\theta}$ with joint regressor for joint positions, but easily cause the foot sliding for the global position prediction.
%
To end this, KIT xx TEMOS~\cite{petrovich22temos}, Language2Pose~\cite{ahuja2019language2pose}, and ~\cite{xx} employ xx named MMM format.
%
Meanwhile, HumanML3D~\cite{Guo_2022_CVPR_humanml3d} \cx{is inspired by} \cite{2021-TOG-AMP} to employ xx with excessive motion features.
%
While all above motion representation in our synthesis framework is optional, we employ xx~\cite{humanml3d} in most experiments to avoid foot sliding issue.





Motion generation, as mentioned, can support rich inputs of multi-modal data, and thus produces various tasks with different conditions.
%
Generally, \textbf{unconditional motion generation}~\cite{temos-57,64,62, mdm2022human} is a more universal task, which models the entire motion space, needs only motion data without any requirement of annotation, and  benefits other generation tasks.
% like AMASS~\cite{AMASS_ICCV2019} dataset, which provide more fora, which is an extremely large motion database unifying many other optical MoCap datasets.
%
We thus evaluate this task on the motion part of \textbf{HumanML3D}~\cite{Guo_2022_CVPR_humanml3d}, which 
provides 14,616 motion sequences from AMASSS~\cite{AMASS_ICCV2019} dataset and 44,970 sequence-level description annotation.
%
For \textbf{text-to-motion} task, we compare with other approaches on two datasets, HumanML3D and \textbf{KIT}, and the latter provides 6353 textual descriptions for 3911 motions.
%
As suggested by \cite{Guo_2022_CVPR_humanml3d}, we use the redundant motion representation in a combination of joint velocities, positions and rotations, which is also used in MDM~\cite{mdm2022human}.
%
\cx{In addition, \cite{action-to-motion} task needs the action-condition motion, similar to the data for action recognition tasks, we thus leverage HumanAct12~\cite{xx} and UESTC~\cite{xx} for evaluation.










==> sections/discussion.tex <==
\section{Discussion}

==> sections/overview.tex <==
% \section{Overview}
% refer to stable diffusion 3.method
% https://arxiv.org/pdf/2112.10752.pdf
